iEdit: Localised Text-guided Image Editing with Weak Supervision

Diffusion models (DMs) can generate realistic images with text guidance using large-scale datasets. However, they demonstrate limited controllability in the output space of the generated images. We propose a novel learning method for text-guided image editing, namely \texttt{iEdit}, that generates images conditioned on a source image and a textual edit prompt. As a fully-annotated dataset with target images does not exist, previous approaches perform subject-specific fine-tuning at test time or adopt contrastive learning without a target image, leading to issues on preserving the fidelity of the source image. We propose to automatically construct a dataset derived from LAION-5B, containing pseudo-target images with their descriptive edit prompts given input image-caption pairs. This dataset gives us the flexibility of introducing a weakly-supervised loss function to generate the pseudo-target image from the latent noise of the source image conditioned on the edit prompt. To encourage localised editing and preserve or modify spatial structures in the image, we propose a loss function that uses segmentation masks to guide the editing during training and optionally at inference. Our model is trained on the constructed dataset with 200K samples and constrained GPU resources. It shows favourable results against its counterparts in terms of image fidelity, CLIP alignment score and qualitatively for editing both generated and real images.

==> experiments_backup.tex <==
\section{Experiments}
\label{sec:experiments}

\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{figs/fig4_generated.pdf}
\end{center}
   \caption{\textbf{Comparison to state-of-the-art on generated images.} Our method produces results with higher fidelity to the input image and the edit prompt compared to SDEdit~\cite{meng2022sdedit}, DALL-E 2~\cite{DALLE2} and InstructPix2Pix~\cite{InstructPix2Pix}.}
\label{fig:qual_gen}
\end{figure*}

In this section, we perform a thorough comparison of \texttt{iEdit} with state-of-the-art methods by quantitative and qualitative analysis on generated and real source images. 

\subsection{Experimental Setup}
\label{ssec:experimentalsetup}

\paragraph{Training Setting.} We use the LDMs~\cite{rombach2022sd} pre-trained on LAION-5B~\cite{schuhmann2022laionb} with the Stable Diffusion checkpoint v1.4\footnote{\url{https://github.com/CompVis/stable-diffusion}}.
We fine-tune \texttt{iEdit} for ${\sim}{10,000}$ steps on 2 16GB NVIDIA Tesla V100 GPUs for $385 \times 384$ resolution with a batch size of 1 and a learning rate of $2\times10^{-4}$. 
To effectively fine-tune on such constrained computational setup, we update the input and middle layers of the UNet in an alternate way. 
Following~\cite{tumanyan2022plugandplay, diffedit}, we set the classifier-free guidance scale to $7.5$.
Inference for $4$ possible editing results per image takes around ${\sim}10$ seconds. 

\vspace{-2mm}\paragraph{Datasets.} We fine-tune \texttt{iEdit} with the paired dataset constructed from LAION-5B~\cite{schuhmann2022laionb} as described in Sec.~\ref{sec:paireddataset}. 
For evaluation with generated images, we use LDM~\cite{rombach2022sd} to construct $70$ image-prompt pairs, with $20$ distinct generated images. 
For evaluation with real images, we build $52$ image-prompt pairs consisting of $30$ distinct images from COCO~\cite{lin2014coco}, ImageNet~\cite{deng2009imagenet} and AFHQ~\cite{choi2020stargan}.

\vspace{-2mm}\paragraph{Comparison to Other Methods.} 
We compare to the SDEdit~\cite{meng2022sdedit} extension of Stable Diffusion since we use a similar diffusion process.
We compare with recent state-of-the-art methods, such as DALL-E 2\footnote{Web UI accessed in March 2023: \url{https://openai.com/product/dall-e-2}.}~\cite{ramesh2022dalle} and InstructPix2Pix\footnote{Web UI accessed in March 2023: \url{https://huggingface.co/spaces/timbrooks/instruct-pix2pix}.}~\cite{InstructPix2Pix}. 
In order to adapt DALL-E 2 for image editing, we manually provide ground-truth masks to each test image during evaluation. 
% To show the impact of different contributions of our proposed approach, we perform an ablation study.
%Additionally, we also compare our method to the global CLIP loss added version of SD and further ablated settings of our proposed method to analyse the contributions of each component.

\vspace{-2mm}\paragraph{Evaluation Metrics.} 
In text-based image editing, we have to evaluate with respect to two dimensions: 1) how well the method synthesises the regions of the image explicitly mentioned in the edit prompt and 2) the quality of preservation of the rest of the image not mentioned in the prompt.
We adapted the Structural Similarity Index (SSIM)~\cite{wang2004ssim} to capture this intuition as: the SSIM score on the edited area (SSIM-$M$) and on the rest of the image (SSIM-$\overline{M}$) by using predicted masks.
In addition, we use CLIPScore~\cite{hessel2021clipscore} to measure the alignment between the edit prompt and the edited image by computing the cosine similarity between their embeddings generated by the CLIP model. 
CLIPScore has been shown in~\cite{EditBench} to be reliable due to its high agreement with human judgement.
We compute the Fréchet Inception Distance (FID)~\cite{seitzer2020fid} to evaluate the quality and fidelity of generated images.
Finally, we visually compare the results of our method with other baselines.


\subsection{Qualitative Evaluation}

\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{figs/fig5_real.pdf}
\end{center}
   \caption{Qualitative Results on Real Images.}
\label{fig:qual_real}
\end{figure*}


\paragraph{Editing Generated Images.} 
Fig.~\ref{fig:qual_gen} compares  \texttt{iEdit} (our method) and \texttt{iEdit}-$M$ (with predicted masks at inference) with SDEdit~\cite{meng2022sdedit}, DALL-E 2~\cite{ramesh2022dalle}, InstructPix2Pix~\cite{InstructPix2Pix} on the generated images as explained in Sec.~\ref{ssec:experimentalsetup}. 
We observe that SDEdit~\cite{meng2022sdedit} fails to perform the desired edit, e.g., \textit{"laughing cat"} in col.~4, \textit{"river"} in col.~7.
It also does not preserve fidelity, e.g., background in \textit{"ship in the sea"} in col.~6 and attributes of the bird in col.~9. 
This is due to SDEdit's trade-off between preservation of the input and editing according to the edit prompt. 
DALL-E 2~\cite{ramesh2022dalle} shows better fidelity to the edit prompt, but it ignores the prior information regarding the object to edit from the source image.
It produces results that completely replace the edited object with a visually different one, e.g. \textit{"sports car"} in col.~2 and \textit{"strawberry cake"} in col.~1. 
The user-provided masks in DALL-E 2 help localising the edit, but its in-painting nature ignores the structure of the edited region from the source images. 
Furthermore, this causes the cases that do not blend well with the general structure of the image, e.g. the tale and wings of the bird in col.~9 and the legs of the astronaut in col.~10 look unrealistic. 
InstructPix2Pix displays high fidelity to both input image and edit prompt, however, it affects the whole layout, e.g. \textit{"a vintage car"} in col.~3 produces a vintage-style image (including background), and the image in col.~8 results in dots.
This is a limitation~\cite{tumanyan2022plugandplay} inherited from Prompt-to-Prompt~\cite{prompt-to-prompt}, used for generating the training set for InstructPix2Pix. 
Compared to these methods, \texttt{iEdit} performs more successful localised edits, while preserving the background, with small undesired changes. 
This is alleviated with the use of predicted masks in \texttt{iEdit}-$M$ at inference.

\vspace{-2mm}\paragraph{Editing Real Images.} 
One of the main advantages of our method is the ability to edit real images without inversions.
Fig.~\ref{fig:qual_real} shows a qualitative comparison on the test set of real images mentioned in Sec.\ref{sec:experiments}.
In accordance with the observations on editing generated images, SDEdit~\cite{meng2022sdedit} achieves low fidelity to edit prompt or source image, e.g., edits in \textit{"pizza"} in col.~1 and \textit{"strawberry prints"} on col.~4, or high deviation from the source image, e.g., \textit{"red tulips"} in col.~5 and \textit{"a cherry tree"} in col.~6. 
DALL-E 2~\cite{ramesh2022dalle} yields results that are inconsistent with the source or look unnatural, e.g. \textit{"wooden house"} in col.~3 and \textit{"white teddy bear wearing blue clothes"} in col.~9. 
The limitation of InstructPix2Pix~\cite{InstructPix2Pix} produces results not complying with the style of the source image (\textit{"bag with strawberry prints"} in col.~4) or affecting the whole image (\textit{"cherry tree"} in col.~6). 
It also fails when multiple changes are requested at once, e.g. \textit{"white teddy bear wearing blue"} in col.~9. 
\texttt{iEdit} shows high fidelity on the source image and the edit prompt on real images as well, where undesired background changes are averted with the introduction of masks in \texttt{iEdit}-$M$.
\begin{table*}[t]
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \small
        \resizebox{\linewidth}{!}{
        \begin{tabular}{ccccc}
         \toprule[0.5pt] 
         \textbf{Method} & \textbf{CLIPScore (\%) $\uparrow$} & \textbf{FID$\downarrow$} & \textbf{SSIM-$M (\%) $} & \textbf{SSIM-$\overline{M}(\%) \uparrow$}\\
         \midrule[0.5pt]
    
         SDEdit & 62.58 & 171 & 69.46 & 68.09 \\ 
         DALL-E 2 & 65.44 & 143 & {80.63} & \textbf{98.04}  \\
         InstructPix2Pix & 65.12 & \textbf{108} & {84.41}  & 87.10 \\
         \hline
         \texttt{iEdit} (ours) & \underline{65.76} & 158 & 70.72 & 68.53 \\
         \texttt{iEdit}-$M$ (ours) & \textbf{66.36} & \underline{114} & 71.53 & \underline{92.83} \\
         
         \bottomrule[0.5pt] 
    \end{tabular}
    }
    \caption{Results on generated images using LDM~\cite{rombach2022sd}.}

    \label{tab:quantitative_results_fake}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.45\textwidth}
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
         \toprule[0.5pt] 
        \textbf{Method} & \textbf{CLIPScore (\%) $\uparrow$} & \textbf{FID$\downarrow$} & \textbf{SSIM-$M (\%)$} & \textbf{SSIM-$\overline{M}(\%) \uparrow$}\\
         \midrule[0.5pt]
    
         SDEdit &  65.84 & 180 & 67.35 & 73.57 \\ 
         DALL-E 2 & 65.46 & 162 & {73.62} & \textbf{97.20}  \\
         InstructPix2Pix & 66.91 & \textbf{145} & {77.77} & 85.17 \\
         \hline
         \texttt{iEdit} (ours) & \underline{67.02} & 166 & 68.11 & 78.68  \\
         \texttt{iEdit}-$M$ (ours) & \textbf{67.44}  & \underline{147} & 69.66 & \underline{87.93}  \\
         
         \bottomrule[0.5pt] 
    \end{tabular}
    }
    \caption{Results on real images from COCO~\cite{lin2014coco}, ImageNet~\cite{deng2009imagenet} and AnimalFaces-HQ~\cite{choi2020stargan}. }
    \label{tab:quantitative_results_real}
     \end{subtable}
     \caption{
     Quantitative results on (a) generated and (b) real images. Best numbers are marked in \textbf{bold}, second best \underline{underlined}.}
     \label{tab:temps}
\end{table*}
\begin{table*}[t]
    \centering
    \footnotesize
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{cc|cccc}
     \toprule[0.5pt] 
     \multicolumn{2}{c}{\textbf{Ablation Settings}} & \multicolumn{4}{c}{\textbf{Scores}} \\
     \textbf{Losses} & \textbf{Fine-tuning Dataset} &   \textbf{CLIPScore (\%) $\uparrow$} & \textbf{FID$\downarrow$} & \textbf{SSIM-$M (\%)$} & \textbf{SSIM-$\overline{M}(\%) \uparrow$}\\
     \midrule[0.5pt]

     % - & \xmark & \xmark &  \xmark & \cmark & \xmark &64.16 & 157 & 70.22 & 67.36 \\ 
      $\mathcal{L}_{global} + \mathcal{L}_{pairs}$  & LAION-caption-200K &  65.95 & 158 &  70.24 & 65.74 \\
     $\mathcal{L}_{global} + \mathcal{L}_{LDM}$+$\mathcal{L}_{loc}$ &LAION-edit-200K    & 65.62 & 156 & 71.23 & 72.57 \\
     $\mathcal{L}_{global} + \mathcal{L}_{LDM}$+$\mathcal{L}_{loc}$+$\mathcal{L}_{perc}$ &LAION-edit-200K   & 65.64 & 153 &  71.46 & \underline{72.64}  \\
      $\mathcal{L}_{global} + \mathcal{L}_{mask}$+$\mathcal{L}_{loc}$+$\mathcal{L}_{perc}$ &LAION-edit-200K  &  \underline{66.09} & \underline{146} & 71.04 & {69.96} \\
      $\mathcal{L}_{global} + \mathcal{L}_{mask}$+$\mathcal{L}_{loc}$+$\mathcal{L}_{perc}$ +Masked Inference &LAION-edit-200K  & \textbf{66.97} &  \textbf{128} & 72.22 & \textbf{87.56} \\
     
     \bottomrule[0.5pt] 
    \end{tabular}
    }
    \caption{Ablation study of \texttt{iEdit} on our loss functions and datasets.}
    \label{tab:quantitative_ablation}
\end{table*}
\vspace{-2mm}
\subsection{Quantitative Evaluation}
Table~\ref{tab:quantitative_results_fake} shows a comparison of state-of-the-art methods and \texttt{iEdit} for editing generated images in our evaluation set. 
In terms of CLIPScore, \texttt{iEdit}-$M$ outperforms all compared methods, which means high alignment and fidelity between the generated and the edit prompt.
\texttt{iEdit}-$M$ is better by $+3.78\%$ and $+1.24\%$ compared to SDEdit and InstructPix2Pix, respectively.  
CLIPScore is one of the main metrics for editing, since it was shown to have high agreement with human judgement~\cite{EditBench}.
We further measure FID, where our method is the second best and is marginally outperformed by InstructPix2Pix.

As SSIM-$M$ measures the SSIM score of the edited area, its high values do not imply a better result, because the edited area could be too similar to that of the source image.
In editing, we want the SSIM-$M$ to be a trade-off between changing the source image accordingly to the edit prompt and not changing it drastically.
So, we attribute the high SSIM-$M$ of DALL-E 2 to the fact that generated images are too similar to source images and might indicate that the editing was not fully successful.
The lower values for SDEdit, \texttt{iEdit} and \texttt{iEdit}-$M$ suggests that they are editing more the source image, confirmed by the results in Fig.~\ref{fig:qual_gen} and~\ref{fig:qual_real}. 
In terms of preserving unrelated parts of images, e.g. the background, DALL-E 2 shows the best SSIM-$\overline{M}$ while \texttt{iEdit}-$M$ has the second best result.
It is worth noting that DALL-E 2 has an unfair advantage in our experiments, since it uses manually-provided masks at inference.
\texttt{iEdit}-$M$ outperforms all other compared methods while relying on predicted masks and gets close to DALL-E 2 (ground-truth masks). 


% \begin{table}[t]
% %\vspace*{-0.3in}
%     \centering
%     \small
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccccc}
%      \toprule[0.5pt] 
%      \textbf{Method} & \textbf{CLIPScore (\%) $\uparrow$} & \textbf{FID$\downarrow$} & \textbf{SSIM-$M (\%) $} & \textbf{SSIM-$\overline{M}(\%) \uparrow$}\\
%      \midrule[0.5pt]

%      SDEdit & 62.58 & 171 & 69.46 & 68.09 \\ 
%      DALL-E 2 & 65.44 & 143 & {80.63} & \textbf{98.04}  \\
%      InstructPix2Pix & 65.12 & \textbf{108} & {84.41}  & 87.10 \\
%      \hline
%      \texttt{iEdit} (ours) & \underline{65.76} & 158 & 70.72 & 68.53 \\
%      \texttt{iEdit}-$M$ (ours) & \textbf{66.36} & \underline{114} & 71.53 & \underline{92.83} \\
     
%      \bottomrule[0.5pt] 
%     \end{tabular}
%     }
%     \caption{Quantitative results on generated images using LDM~\cite{rombach2022sd}. Best numbers are marked in \textbf{bold}, second best \underline{underlined}.}

%     \label{tab:quantitative_results_fake}
% \end{table}

% \begin{table}[t]
% %\vspace*{-0.3in}
%     \centering
%     \small
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccccc}
%      \toprule[0.5pt] 
%     \textbf{Method} & \textbf{CLIPScore (\%) $\uparrow$} & \textbf{FID$\downarrow$} & \textbf{SSIM-$M (\%)$} & \textbf{SSIM-$\overline{M}(\%) \uparrow$}\\
%      \midrule[0.5pt]

%      SDEdit &  65.84 & 180 & 67.35 & 73.57 \\ 
%      DALL-E 2 & 65.46 & 162 & {73.62} & \textbf{97.20}  \\
%      InstructPix2Pix & 66.91 & \textbf{145} & {77.77} & 85.17 \\
%      \hline
%      \texttt{iEdit} (ours) & \underline{67.02} & 166 & 68.11 & 78.68  \\
%      \texttt{iEdit}-$M$ (ours) & \textbf{67.44}  & \underline{147} & 69.66 & \underline{87.93}  \\
     
%      \bottomrule[0.5pt] 
%     \end{tabular}
%     }
%     \caption{Quantitative results on real images from COCO~\cite{lin2014coco}, ImageNet~\cite{deng2009imagenet} and AnimalFaces-HQ~\cite{choi2020stargan} images. Best numbers are marked in \textbf{bold}, second best \underline{underlined}.}

%     \label{tab:quantitative_results_real}
% \end{table}

In Table~\ref{tab:quantitative_results_real}, we present a quantitative evaluation of our method and compared methods on editing the real images in our evaluation set. 
We observe a similar trend to the results obtained on generated images (Table~\ref{tab:quantitative_results_fake}). 
As before, even without using masks at inference, our method produces results with higher fidelity to the edit prompt in terms of CLIPScore. 
Conclusions similar to the case of generated images can be drawn for FID, SSIM-${M}$ and SSIM-$\overline{M}$.

\subsection{Ablation Study}
We validate the effectiveness of each component of \texttt{iEdit} by an ablation study on the full evaluation set (generated and real images), summarised in Table~\ref{tab:quantitative_ablation}.
First, we compare LAION-caption-200K (first row) and LAION-edit-200K ($2^{nd}$ row).
LAION-edit-200K is the dataset constructed as described in Sec.~\ref{sec:paireddataset} with BLIP-generated edit prompts, used as fine-tuning set in all previous experiments.
LAION-caption-200K is created in the same way but using the original captions instead of the automatically-generated ones. 
We use the best experimental setup for LAION-caption-200K, which employs $\mathcal{L}_{global} + \mathcal{L}_{pairs}$.
Because, the difference between these noisy source and target captions of LAION-5B are too high (even different languages sometimes) and often not grounded to images.
This prevents the use of masks $\mathcal{L}_{mask}$ and of $\mathcal{L}_{perc}$ and $\mathcal{L}_{loc}$.
% Since the original captions are noisy, manipulating a word does not produce meaningful results. Therefore, we use the embedding of the source caption when fetching the nearest neighbour. Furthermore, the difference between these noisy source and target captions are not meaningful which prevent the use of masks and therefore the use of $\mathcal{L}_{perc}$ and $\mathcal{L}_{loc}$.
The $1^{st}$ and $2^{nd}$ row of Table~\ref{tab:quantitative_ablation} show benefit of automatically-generated prompts with higher CLIPScore and SSIM-$\overline{M}$.

Moreover, we ablate our main losses and components forming the masked image editing framework, by training only with the localised CLIP loss $\mathcal{L}_{loc}$ ($2^{nd}$ row), by adding $\mathcal{L}_{perc}$ ($3^{rd}$ row) and by switching $\mathcal{L}_{LDM}$ in favour of $\mathcal{L}_{mask}$ ($4^{th}$ row). 
The addition of $\mathcal{L}_{perc}$ marginally boosts the performance in all metrics,  while $\mathcal{L}_{mask}$ leads to a large improvement in CLIPScore and FID.
%Although background preservation decreases, introducing masked inference results in significant increase in all metrics.
The final row of Table~\ref{tab:quantitative_ablation} 
(predicted masks at inference) shows a large improvement in all metrics.
